Analysis of a Gray-Box Operator for Vertex Cover

Combinatorial optimization problems are a prominent application area of evolutionary algorithms, where the (1+1) EA is one of the most investigated. We extend this algorithm by introducing some problem knowledge with a specialized mutation operator which works under the assumption that the number of 1s of a solution is critical, as frequently happens in combinatorial optimization. This slight modification increases the chance to correct wrongly placed bits while preserving the simplicity and problem independence of the (1+1) EA. As an application of our algorithm we examine the vertex cover problem on certain instances, where we show that it leads to asymptotically better runtimes and even finds with higher probability optimal solutions in comparison with the usual (1+1) EA. Precisely, we compare the performance of both algorithms on paths and on complete bipartite graphs of size $n$. Regarding the path we prove that, for a particular initial configuration, the \alg1+1 takes in expectation $\Theta(n^4)$ iterations while the modification reduces this to $\Theta(n^3)$, and present experimental evidence that such a configuration is reached. Concerning the complete bipartite graph our modification finds the optimum in polynomial time with probability $1-1/2^{\Omega(n^\xi)}$ for every positive constant $\xi < 1$, which improves the known probability of $1-1/\text{poly}(n)$ for the (1+1) EA..

==> probForbipartite_one_plus_one_EA.tex <==
%!TEX root = balanced_EA_vertex_cover.tex

\begin{theorem}
	\label{theorem::poly_and_exp_time_one_one_EA}
	Let $B=(V_L \cup V_R,E)$ be a complete bipartite graph instance of the Vertex Cover Problem, where $L:=|V_L|$, $R:=|V_R|$, $n:=R+L$, and $c:=R/L \geq 2$. 
	After a polynomial number of iterations of the \alg1+1 with fitness $f$, we have a probability of at least $\frac{1}{\text{poly}(n)}$ 
	obtaining a stage where all vertices in $V_R$ are selected while no vertex in $V_L$ is selected.
	Moreover, leaving this stage after a polynomial number of steps has probability of at most $\frac{1}{\text{exp}(n)}$. 
\end{theorem}

\begin{proof}
	For the first part of the lemma we separate the proof into two phases.
	The first phase is to give a lower bound on the probability that $V_R$ is completely selected by the \alg1+1 after $12en\ln n$ iterations,
	and the second phase is to give a lower bound on the probability that all selected vertices becomes unselected after additional $n^{3/2}$ iterations under the assumption that the first phase is already successfully executed.
	For the second part of the lemma we prove coming out of this resulting local optimum after a polynomial number of iterations has at most exponentially decreasing probability in $n$. 
		
	We define a \textit{simple $V_R$-step} as a step where only one bit in $V_R$ is flipped and no other.
	This probability is 
	$\frac{R}{R+L} \cdot \left(1- \frac{1}{R+L}\right)^{R+L-1} \geq \frac{c}{e(c+1)} \geq \frac{2}{3e}$ as $c\geq2$.
	Let $Y$ be the random variable which describes the number of iterations of the \alg1+1 until $k \cdot \frac{2}{6e} = \frac{k}{3e}$ simple $V_R$-steps are executed.
	$Y$ is geometrically distributed with probability at least $\frac{2}{3e}$ and hence one execution of a $V_R$-step takes in expectation $\frac{3e}{2}$ iterations and therefore $E[Y] = k \cdot \frac{2}{6e} \cdot \frac{3e}{2} = \frac{1}{2} k$.
	By using Markov's inequality we obtain for $k-1$ iterations of the \alg1+1 a probability of $P[Y < k] = 1-P[Y \geq k] \geq 1/2$ having at least $\frac{k}{3e}$ simple $V_R$-steps.
	Thus, setting $k=12en\ln n$ leads to $4 n \ln n$ simple $V_R$-steps with probability of at least $1/2$.
	
	Next, we make use of the multiplicative drift \cref{theorem::multiplicative_drift} to compute an expected running time until all vertices of $V_R$ are selected through simple $V_R$-steps to obtain a lower bound on the probability to get that stage after $12en\ln n$ iterations of the \alg1+1.
	We denote such a vertex cover (or stage) as a $V_R$-cover.
	All of our following computations are based under the assumption that $V_L$ was never completely selected during this time.
	Let $N$ be the current weight number of uncovered edges.
	Every simple $V_R$-step that flips a zero to a one is accepted and vice versa rejected by the fitness $f$.
	Thus, the latter contributes a weight decrease of zero.
	The total weight decrease of those simple $V_R$-steps is $N$ as selecting $V_R$ corresponds to a valid vertex cover.
	Therefore, we get for an accepted $V_R$-step an expected weight decrease of $N$ by a factor of $1-1/R$.
	Let $Z_i$ be the random variable describing the current weight $N$ after $i$ simple $R$-steps.
	Note that $N \leq n^2$, and that $Z<1$ is equivalent to that we produced a $V_R$-cover.
	By the explanations above we have $V_R$-step iteration wise an expected multiplicative drift decrease of 
	$$E[Z_{i} - Z_{i+1} \mid Z_{i} = k \geq 1] \geq k - k (1-1/R) \geq 1/n.$$
	Thus, using \cref{theorem::multiplicative_drift} with $\delta = 1/n$, $s_0 = n^2$ and $s_{\min} = 1$ yields to an expected waiting time of at most $2n \ln n + n \leq 3 n \ln n$ simple $V_R$-steps to obtain a $V_R$-cover.
	Let $T$
	%= \inf \{Z \in \R_{\geq 0} \mid Z <1\}$
	be defined as this hitting time.
	By Markov's inequality we obtain $P[T <  4 n \ln n] = 1 - P[T \geq 4 n \ln n] \geq 3/4$.
	As a result, we obtain a $V_R$-cover after $4 n \ln n - 1$ $V_R$-steps with probability at least $3/4$ and therefore, with probability at least $1/2 \cdot 3/4 = 3/8$ a $V_R$-cover after $12en\ln n$ iterations of the \alg1+1.
	
	Further, we compute a lower bound on the probability that at least one vertex in $V_L$ is unselected after $12 n \ln n$ iterations of the \alg1+1.
	We base the analysis of the assumption that after $12 n \ln n$ iterations $V_R$ is completely selected.
	Note that this assumption does not decrease the probability of an unselected vertex from $V_L$.
	By Chernoff bounds, there are with probability $1-2^{-\Omega(L)}$ at least $L/3 = n^{\delta}/3$ vertices of $V_L$ unselected in a u.a.r.~initial solution for a $\delta \in (0,1)$.
	The probability that after $12en \ln n$ iterations of the \alg1+1 a single vertex is
	chosen at least once is $1-(1-1/n)^{12en \ln n}$ and therefore, the probability that at least one of the initially unselected vertices of $V_L$ is still unselected after $12en \ln n$ iterations is $1 - (1-(1-1/n)^{12en \ln n})^{n^{\delta}/3}$
	which is roughly estimated at least $n^{\delta - 13 e}/6$.
	
	We approximate now the probability under the assumption that the events,
	\begin{itemize}
		\item  producing a $V_R$-Cover after $12en \ln n$ iterations of the \alg1+1, and 
		\item  that during this time there is still at least one unselected vertex in $V_L$,
	\end{itemize}
	are independent.
	As a result, the desired state space occurs with probability of at least $ \frac{3}{8} \cdot  \frac{n^{\delta - 13 e}}{6} = \frac{n^{\delta - 13 e}}{16}$ for a $\delta \in (0,1)$.
	Note that the approximation is justified since we wish to have a probability of at least $\frac{1}{\text{poly}(n)}$.%, where $L=\frac{1}{c+1} n$ for the ratio $c=R/L$.
	
	Remains to show that all selected vertices in $V_L$ becomes unselected.
	Pessimistacally, we assume that except of one all vertices in $V_L$ are selected.
	We distinguish between the events
	\begin{itemize}
		\item[(a)] all missing vertices of $V_L$ and at least as many vertices of $V_R$ are flipped, and
		\item[(b)] all vertices of $V_R$ stays untouched and the number of selected vertices in $V_L$ is decreased or stays the same by flipping some selected and unselected vertices in $V_L$.
	\end{itemize}
	Note that all other mutations will be rejected by the fitness $f$.
	For (a) we have probability of at most $n^{-k}$, where $k$ denotes the current number of unselected vertices in $V_L$.
	For (b) we restrict ourself to 1-bit-flips reducing the number of selected vertices in $V_L$ and thus, the probability is at least $\frac{L-k}{n} \cdot (1-1/n)^{n-1} \geq \frac{L-k}{en} \geq \frac{1}{en}$.
	Note that all other mutation steps reduce or preserves the number of selected vertices in $V_L$.
	The probability that (b) occurs before (a) is  $\frac{1}{en}/\left(\frac{1}{en} + n^{-k}\right) = 1 - \frac{e}{n^{k-1}+e}$.
	As a result, the probability that only the vertices in $V_R$ are selected before the event (a) occurs is at least
	
	$$\prod_{k=1}^{L-1} \left(1- \frac{e}{n^{k-1}+e} \right)  \geq \frac{1}{1+e} \left(1 - \frac{e}{n}\right)^{(n-1)/2} \geq \frac{e^{-e/2}}{1+e} > \frac{1}{15}.$$
	
	The expected waiting time that all vertices in $V_L$ becomes unselected is in $\O(n\log n)$, which for example might be proved by using the multiplicative drift theorem.
	Let $T$ be this hitting time.
	Under the assumption that event (a) not occurs after $n^{3/2}-1$ iterations, we obtain $P[T < n^{3/2}] = 1 - P[T \geq n^{3/2}] \geq 1-\frac{\O(n \log n)}{n^{3/2}}$ by using Markov's inequality,
	which gives a probability of $1-o(1)$ that all vertices in $V_L$ becomes unselected after $n^{3/2}$ iterations. 
	As a result, we obtain for a $\delta \in (0,1)$ a probability of at least $\frac{n^{\delta - 13 e}}{16} \cdot \frac{1}{15} = \frac{n^{\delta - 13 e}}{240}$ a stage in the \alg1+1 that the vertices in $V_R$ are completely selected while no vertex in $V_L$ is selected, which is greater than $\frac{1}{\text{poly}(n)}$. %as $L=\frac{1}{c+1}n$ for the assumed constant ratio $c=R/L$.
	
	
	The second part of the lemma can simply proven in the following way: leaving the above given stage has probability of at most $n^{\Omega(-L)} = n^{\Omega\left(-\frac{n}{c+1}\right)}$.
	Thus, such an event happens in expectation after an exponential number of iterations of the \alg1+1.
	That is, we obtain a probability of $\frac{1}{\text{exp(n)}}$ that this event happens after a polynomial number of iterations. 
\end{proof}

\begin{theorem}
	Let $B=(V_L \cup V_R,E)$ be a complete bipartite graph instance of the Vertex Cover Problem, where $L:=|V_L|$, $R:=|V_R|$, $n:=R+L$, and $c:=R/L \geq 2$. 
	After a polynomial number of iterations of the \alg1+1 with fitness $f$, we have a probability of $1-\frac{1}{poly(n)}$ finding the optimal solution.
\end{theorem}
\begin{proof}
	We consider two events:
	\begin{itemize}
		\item[A] There will be a stage during the algorithm, where every vertex in $V_R$ is selected while no vertex in $V_L$ is selected.
		\item[B] The algorithm finds after a polynomial number of steps the optimum.
	\end{itemize}
	We make use of the law of total probability and \cref{theorem::poly_and_exp_time_one_one_EA} to obtain
	\begin{align*}
		P[B] &= P[B \text{ and } A] + P[B \text{ and } \neg A]\\
		&=	P[B \text{ and } A] + P[B \mid A] \cdot P[A]\\
		&\leq  P[\neg A] + P[B \mid A]\\
		&\leq 1 - \frac{1}{\text{poly}(n)} + \frac{1}{\text{exp}(n)} 
	\end{align*}
	The resulting term is clearly dominated by $1 - \frac{1}{\text{poly}(n)}$, which proves the Theorem.
\end{proof}

